Irrational l2-invariants arising from the lamplighter group

We show that the Novikov-Shubin invariant of an element of the integral group ring of the lamplighter group Z_2 \wr Z can be irrational. This disproves a conjecture of Lott and Lueck. Furthermore we show that every positive real number is equal to the Novikov-Shubin invariant of some element of the real group ring of Z_2 \wr Z. Finally we show that the l2-Betti number of a matrix over the integral group ring of the group Z_p \wr Z, p>1, can be irrational, and so the groups Z_p \wr Z become the simplest known groups which give rise to irrational l2-Betti numbers.

==> coaster-intro.tex <==
%\section{Introduction}
\vspace{5pt}
Let $\Ga$ be a countable discrete group. A real number $r$ is said to be an
\textit{$l^2$-Betti number arising from $\Ga$} if there is a matrix $T$ with entries in the integral group ring $\Z [\Ga]$, such that the \textit{von Neumann dimension} of the kernel of $T$ is equal to $r$. 

The motivation for the name is as follows: when  $r$ is an $l^2$-Betti number arising from $\Ga$, then there exists a normal covering $M$ of a finite CW-complex whose deck transformation group is $\Ga$, and such that one of the $l^2$-Betti numbers of $M$ is equal to $r$.  We refer to the very readable introduction \cite{Eckmann_intro} for more details.

The following problem is a fine-grained version of a question asked by Atiyah in \cite{Atiyah1976}.

\begin{problem}[The Atiyah problem for $\Ga$] What is the set of $l^2$-Betti numbers arising from $\Ga$?
\end{problem}
Let us denote this set by $\cal C(G)$. For a class of groups
$C$ define $\cc C(C) = \cup_{\Ga\in C} \cc C(\Ga)$. 

So far $\cc C(\Ga)$ has been computed only in cases where $\cc C(\Ga)$ turns out to be a subset of $\Q$. In fact, the statement  known as the \textit{Atiyah conjecture for torsion-free groups} says that $\cc C(\Ga)=\N$ for any
torsion-free group, and before \cite{Dicks_Schick} it was widely conjectured that $\cc C(\Ga) \subset \Q$ for every group $\Ga$. However, \cite{Dicks_Schick} gives an example of a group ring element  $T$ together with an heuristic argument showing why the von Neumann dimension of $\ker T$ is probably irrational. That example is based on \cite{Grigorchuk_Zuk2001}, where a weaker form of the Atiyah conjecture was disproved.

Only recently Austin \cite{arxiv:austin-2009} obtained  a definite result by proving 
that $\cc C($Finitely generated groups$)$ is uncountable.  His results were extended and simplified in  \cite{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem}  and \cite{arxiv:pichot_schick_zuk-2010}, and additional examples were found in  \cite{arxiv:lehner_wagner-2010}.

All the groups $G$ for which it was shown $\cal C(G)\not\subset \Q$ have one of the lamplighter groups $\ZZ_p\wr \ZZ$, $p=2,3\ldots$, as a subgroup for some $p$, but are substantially more complicated than that.

%~ 
%~ That work has been a motivation for much of the
%~ following efforts, in that it showed that  the computation of $\dimvn\ker (T)$ can sometimes be done by analyzing certain
%~ dynamical systems and using the Pontryagin duality. This computation method is explained in Section \ref{sec-tool-basic}. 
%~ that in fact $\cc C($Finitely generated groups$)=\R_{\ge 0}$ and 
%~ $\cc C($Finitely presented groups$)
%~ \nsubseteq \Q$. Moreover, in \cite{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem} it is shown that $\cc C((\Zmod{2}\wr \ZZ)^3)
%~ \nsubseteq \Q$. 
%~ 
%~ More recently, Lehner and Wagner showed in \cite{arxiv:lehner_wagner-2010} that $\cc C(\Zmod{p} \wr
%~ F_d)$ contains irrational algebraic numbers, where $F_d$ is the free group on $d$ generators, $d\ge 2$,  and $p \ge 2d-1$.
%~ 
%~ In all the articles cited above the following is true: if it is proven that for a given group $
%~ \Ga$ we have $\cc C(\Ga)\nsubseteq \Q$, then there exists $p$ such that $\Zmod{p} \wr \ZZ \subset \Ga$. 

Our first result is as follows.

\begin{theorem}\label{thm-intro-zero} There is a matrix $T$ with entries in the group ring $\Z[\ZZ_p\wr\ZZ]$ such that 
$$
\dimvn\ker T = 1344\left( \frac{4p^3+3p^2+2p-1}{8p^3} + \frac1{8p^3} \sum_{k=1}^\infty \left(\frac{p-1}{p}\right)^{k+2^{k}}\right),
$$
which is a transcendental number.
\end{theorem}

In the view of the preceding discussion, the following problem captures the limit of the currently available methods for finding groups $\Ga$ such that $\cal C(\Ga) \not\subset \Q$.

\begin{problem} Does $\cc C(\Ga) \not\subset \Q$ imply $\Zmod{p}\wr \ZZ\subset \Ga$ for some $p$?
\end{problem}


As mentioned above, $\cc C(\Ga)$ has been computed only in the cases where in fact $\cc C(\Ga)\subset \Q$. Since $\ZZ_p\wr\ZZ$ are  the simplest groups for which we know $\cal C(\Ga)\not\subset\Q$, it is natural to ask the following.
%In view of the above, the ``easiest'' group known for which $\cc C(\Ga)\nsubseteq \Q$ is $\Zmod{2}\wr\ZZ$, and hence the following question.

\begin{problem} Is there a description of $\cc C(\Zmod{2}\wr \ZZ)$ substantially different from the definition?
\end{problem}

To state a more concrete problem:  is $\sqrt 2 \in \cc C(\Zmod{2}\wr \ZZ)$ ?

\vspace{5pt}
For our second result let us recall the definition of another spectral invariant associated to an element of a group ring, the \textit{Novikov-Shubin invariant}. It measures the growth of the number of eigenvalues around $0$. More precisely, given a self-adjoint $T\in \C[\Ga]$, the Novikov-Shubin invariant of $T$ is defined as 
\beq\label{eq-ns-def}
\al(T) := \liminf_{\la\to 0^+}\frac{\log(\mu_T((0,\la]))}{\log(\la)},
\eeq
where $\mu_T$ is the spectral measure of $T$ (see \cite[Chapter 2]{Lueck:Big_book} for more details).

\begin{remarks} (i) It is irrelevant whether we take $\mu_T((0,\la])$ or $\mu_T((0,\la))$ in \eqref{eq-ns-def}. However, it is important that we do not include $0$, since otherwise $\al(T)$ would be equal to $0$ whenever the spectral measure of $T$ has an atom at $0$. It is also irrelevant what is the base of the logarithm. It is convenient for us to take the base-$2$ logarithm.

(ii) Both the numerator and the denominator are negative when $\la$ is sufficiently small, so $\al(T) \in [0,\infty]$.

(iii) If for some $d$ and all $\eps$ there is a constant $C>0$ such that for sufficiently small $\la$ we have $\frac1C\la^{d+\eps} < \mu_T((0,\la)) < C\la^{d-\eps}$ then a short computation shows that $\al(T) = d$.
\end{remarks}

Lott and L\"uck \cite{lott-lueck-l2-topological-invariants-of-3-manifolds} proposed the following conjecture.

\begin{conjecture}\label{conj-lott-lueck-intro} When $T\in \Z[\Ga]$ then $\al(T) >0$ and $\al(T)\in \Q$.
\end{conjecture}

For counterexamples to the positivity part see \cite{2014arXiv1409.3212G}. In the present paper we construct $T\in \Z[\ZZ_2\wr \ZZ]$ such that $\al(T)\notin \Q$. In fact we show the following.

\begin{theorem}\label{thm-intro-ns}
There is a family $T(b)\in \R[\ZZ_2\wr\ZZ]$, $b\in (1,\infty)$ such that for $b\in \Q$ we have $T(b)\in \Q[\ZZ_2\wr\ZZ]$ and $\al(T(b)) = \frac1{2\log_2(b)}$.
\end{theorem}

Note that the Novikov-Shubin invariant of $T$ and $kT$ is the same for $k>0$, and so we also obtain examples of $T\in \Z[\ZZ_2\wr\ZZ]$ with  irrational Novikov-Shubin invariants.

To the author's best knowledge, the counterexamples to the rationality part of Conjecture \ref{conj-lott-lueck-intro} were not known before even if $\Z[\Ga]$ is replaced by $\R[\Ga]$. The family $T(b)$ is a modification of the operator studied by Grigorchuk and \.Zuk \cite{Grigorchuk_Zuk2001}.

For partial results and the motivations for Conjecture \ref{conj-lott-lueck-intro} see \cite[Section 2.5]{Lueck:Big_book}. Let us only mention that a good deal of the motivation comes from the concrete computations. As in the case of $l^2$-Betti numbers, when $r$ is a Novikov-Shubin invariant of some $T\in \Z[G]$,  then there exists a normal covering $M$ of a finite CW-complex whose deck transformation group is $\Ga$, and such that one of the Novikov-Shubin invariants of $M$ is equal to $r$. 


\begin{conjecture} The Novikov-Shubin invariants of the universal cover of a closed aspherical CW-complex are positive and rational.
\end{conjecture}

Thereom \ref{thm-intro-ns} has an interesting consequence that the set of the Novikov-Shubin invariants of all the elements of $\Q[\ZZ_2\wr\ZZ]$, which  is countable, is  different than the set of the Novikov-Shubin invariants of all the elements of $\R[\ZZ_2\wr\ZZ]$. The analogous question has been asked among the experts for $l^2$-Betti numbers, since there are classes of torsion-free groups for which the Atiyah conjecture is known for $\Q[\Ga]$ but not for $\R[\Ga]$.

\begin{problem}\label{problem-9}
Is it the case that for every $T\in \R[\Ga]$ there exists $T'\in \Q[\Ga]$ such that $\dimvn\ker T = \dimvn\ker T'$?
\end{problem}

Although Theorem \ref{thm-intro-ns} shows that the answer is negative when we replace $\dimvn\ker T= \dimvn\ker T'$ with $\al(T) = \al(T')$, the author believes that at least for $\Ga= \ZZ_2 \wr \ZZ$ the answer to Problem \ref{problem-9} is positive. 


We finish by mentioning a question first noted in \cite{MR1132295} which seems within the reach of the method used here and in \cite{2014arXiv1409.3212G}. 

\begin{problem}
Can  $\liminf$  be replaced by $\lim$ in the definition of $\al(T)$?
\end{problem}
One of the motivations for this question is that a fundamental property of the Novikov-Shubin invariants, \textit{the product formula} (see \cite[Corollary 2.44]{Lueck:Big_book}), is known to hold in general only under the assumption that the answer is positive.


\vspace{5pt} The structure of the article is as follows. In the next section we describe the computational tool, in a generality which is just enough for the proof of Theorem \ref{thm-intro-ns}. A general version is presented in \cite[Section 2]{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem} and we refer there for the proofs. Various variants of it were also used for example in \cite{MR1436310}, \cite{Dicks_Schick}, \cite{Lehner_Neuhauser_Woess:On_the_spectrum_of},  \cite{arxiv:austin-2009}, and \cite{arxiv:pichot_schick_zuk-2010}.

In Section \ref{sec-ns} we prove Theorem \ref{thm-intro-ns}. Section \ref{sec-tool-non-basic} presents a slightly different version of the computational tool, which is then used in Section \ref{sec-the-operator} to prove Theorem \ref{thm-intro-zero}. 

Some elementary linear algebra computations are deferred to the appendix.

\vspace{5pt}\textbf{Notation.} The rings of integer, rational, real and complex numbers are $\Z$, $\Q$, $\R$ and $\C$. The cyclic group of order $p$ is $\ZZ_p$ and the infinite cyclic group is $\ZZ$. We fix a generator of $\ZZ$ and denote it by $t$. Given an action $\Ga\actson X$, the result of the action of $\ga\in \Ga$ on $x\in X$ is denoted by $\ga.x$. For example the  translation action of $\ZZ\actson \Z$ is, by definition, given by $t.k:=k{+}1$.

\vspace{5pt}\textbf{Note on chronology.} The first version of this article submitted to arXiv in 2010 contained only Theorem \ref{thm-intro-zero}. Theorem \ref{thm-intro-ns} was added in 2014.

\vspace{5pt}\textbf{Thanks.} The author thanks  {\'S}wiatos{\l}aw Gal,  Holger Kammeyer, Jarek K\k{e}dra, Manuel Koehler, Thomas Schick and Andreas Thom for useful comments. 

The author was supported by EPSRC at Imperial College London and Oxford University, by EPSRC grant EP/K012045/1 at University of Warwick, and by Fondations Sciences Math{\'e}matiques de Paris during the program \textit{Marches Al\'eatoires et G\'eom\'etrie Asymptotique des Groupes} at Institut Henri-Poincar\'e.

%~ 
%~ 
%~ Following G. Elek (ref...), For an amenable group $\Ga$ one can study analogs of the kernel von Neumann dimension $\dim_{\Q[\Ga]}\ker(T)$ over arbitrary fields, by taking limits along Foelner sequences. We denote the resulting kernel dimension by $\dim_{\kk[\Ga]}\ker(T)$.
%~ 
%~ Assume the characteristic $q:=\chi(\kk) \ge 3$. Let $r$ be the multiplicative order of $2$ in $\kk$, let $L\subset \{2,3,\ldots \}$ be the set of minimal representatives mod $q$ of the powers $2^i$, $i\ge 1$ and for $x\in L$ let $r(x)$ be the smallest such that $2^{r(x)} =x \mod q$. 
%~ 
%~ \begin{theorem}\label{thm-intro-positive} We have
%~ $$
%~ \dim_{\kk[\ZZ_2\wr\ZZ]} \ker \rho(T) = 1344\cdot (\frac{47}{64} + \frac{1}{128}\scdot \frac{1}{2^r-1} + \frac{1}{64}\scdot \frac{2^q}{2^q-1} \scdot \sum_{x\in L} \frac{1}{2^{x+r(x)-1}}),
%~ %\frac{1}{64}(45+ \frac{1}{2^r -1} + 1 + 2+ 2\sum_{x\in L}\frac{1}{2^{x+r(x)}}\scdot \frac{2^r}{2^r-1}\scdot \frac{2^q}{2^q-1})),
%~ $$
%~ where $\rho(T)\in \kk[\ZZ_2\wr\ZZ]$ is the reduction $\!\!\mod q$ of $T$. 
%~ \end{theorem}
%~ 
%~ Clearly the right hand side above is a rational, since $L$ is a finite set. It has been sometimes informally conjectured that thers should be $q_0$ (depending on $T$) such that if $q \ge q_0$ then
%~ $$
	%~ \dim_{\kk[\ZZ_2\wr\ZZ]} \ker \rho(T)  = \dim_{\Q[\ZZ_2\wr\ZZ]} \ker (T). 
%~ $$ 
%~ It is very easy to see that $\lim_{\chi(\kk)\to\infty} \dim_{\kk[\ZZ_2\wr\ZZ]} \ker \rho(T)  = \dim_{\Q[\ZZ_2\wr\ZZ]}\ker(T)$, and so this conjecture is false:
%~ \begin{cory}
%~ As $\kk$ runs through different fields, $\dim_{\kk[\ZZ_2\wr\ZZ]} \ker (T)$ assumes infinitely many different values.
%~ \end{cory}
%~ 
%~ Given a finite CW-complex $X$ with fundamental group $\Ga$ which is amenable and residually finite, we can define, after (ref...) and (ref...), the $\kk$-homology gradient of $X$, by taking the limit over finite covers of $X$ of the dimensions of $\kk$-homology groups normalized by the index. By (ref...) and (ref...) we get the following corollary.
%~ 
%~ \begin{cory}
%~ There exists a finite CW complex with fundamental group $\ZZ_2\wr \ZZ$ whose  $\kk$-homology gradients in degree $4$ assume infinitely many different values as $\kk$ runs through different dields.
%~ \end{cory}


==> coaster-ns.tex <==
\renewcommand{\0}{\,{\texttt{\large 0}}}
\renewcommand{\1}{\,{\texttt{\large 1}}}
\newcommand{\2}{\,{\texttt{\large 2}}}
\newcommand{\D}{\,{\texttt{\large D}}}
\renewcommand{\-}{\,{\texttt{\small $\bullet$}}}
\newcommand{\ppp}{\,{\texttt{\small $\bullet$}}}
\renewcommand{\u}{\underline}

\section{Computational tool in the case of a free action}\label{sec-tool-basic}

Assume that $(X,\mu)$ is a compact abelian group with the normalized Haar measure which is Pontryagin-dual to a countable discrete abelian group $A$. Assume furthermore that the action $\Ga\actson X$ is by continuous group automorphisms. 
The Pontryagin duality gives us  an embedding $\C[A]\into L^\infty(X)$. The preimage of $f\in L^\infty(X)$ under this embedding, if it exists, is denoted by $\wh f$ (see \cite[Chapter 4]{Folland:A_course_in_abstract_harmonic_analysis} for more on the Pontryagin duality).  

Let $\chi_1,\ldots, \chi_n$ be the indicator functions of subsets $X_1,\ldots, X_n\subset X$ such that all  $\chi_i$ have preimages. Let $a_1,\ldots, a_n\in \C$ and $\ga_1,\ldots, \ga_n \in \Ga$.

Let $\wh T\in \C[\Ga\ltimes A]$ be defined as $\wh T:= \sum a_i\ga_i\wh\chi_i$, and let $T\in\Ga\ltimes  L^\infty(X)$ be defined as $T := \sum a_i\ga_i\chi_i$. As explained for example in \cite[Section 2]{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem}, we have the following lemma.

\begin{lemma}\label{lem-pontryagin}
The spectral measures of $\wh T$ and of $T$ are the same. \qed
\end{lemma}

We will now explain how to compute the spectral measure of $T$ \textit{under the assumption that the action $\Ga\actson X$ is essentially free}, i.e.~there is a subset $X'\subset X$ of full measure which is $\Ga$-invariant and such that the action of $\Ga$ on $X'$ is free.

Consider the oriented edge-labelled graph $\cal G$ defined as follows. The set of vertices of $\cal G$ is $X$, and there is an edge from $x_1$ to $x_2$ if for some $i$ we have $x_1\in X_i$ and $\ga_i.x_1=x_2$. On such an edge we set the label to be equal to 
\def\mathclap#1{\text{\hbox to 0pt{\hss$\mathsurround=0pt#1$\hss}}}
%\limits_{\mathclap{\substack{z\in Z\colon\\ \mu_z(S_\de.U) 
$$
	\sum_{\mathclap{\substack{j\colon \ga_j=\ga_i\\x_1\in X_j}}} a_j.
$$

 Let $\cal G(x)$ be the connected component of $x$ in $\cal G$. Let $l^2(\cal G(x))$ be the Hilbert space spanned by the vertices of $\cal G(x)$. Let $T(x) \colon l^2(\cal G(x)) \to l^2(\cal G(x))$ be the adjacency operator on $\cal G(x)$, i.e.~the entry of the matrix of $T(x)$ corresponding to a pair of vertices $(v_1, v_2)$ is equal to the label on the edge from $v_1$ to $v_2$, if there is such an edge, and $0$ otherwise.

We say $T$ is \textit{self-adjoint} if the set of those $x$ for which the matrix of $T(x)$ is Hermitian is of measure $1$. 

\begin{proposition}\label{prop-tool-free}
Let us assume that $T$ is self-adjoint and that the set of those $x$ for which $\cal G(x)$ is finite is of measure $1$. Then for a measurable subset $D\subset \R$ we have 
$$
\mu_T(D) = \int_X \frac{\mu_{T(x)}(D)}{|\cal G(x)|}\,d\mu(x).
$$\qed
\end{proposition}


We will apply this proposition in the next  section. Its utility comes from the fact that among the labelled graphs $\cal G(x)$, $x\in X$, there are  only countably many different ones, and they can be computed explicitly. As such the above integral will decompose as an explicit countable sum of spectral measures of \textit{finite-dimensional} matrices.

\section{Possible values of the Novikov-Shubin invariants}\label{sec-ns}

We need a more quantitative version of \cite[Lemma 5]{2014arXiv1409.3212G}. For $b\in \R$ and $n\in \N$ let $M(b,n)$ be the $n\times n$ matrix
$$
\left( \begin{array}{cccccc}
1 & b &  &  &   \\
b & b^2+1 & b &   &   \\
 & b & b^2+1  &  &   \\
& & & \ldots & & \\
 & & &  & b^2+1 &b \\ 
  & & &  &b & b^2+1
\end{array} \right)
$$

\begin{lemma}\label{lem-matrix-lemma}
For every $\eps$ and $b>1$ there is $N$ such that for $n>N$ the matrix $M(b,n)$ has an eigenvalue $\la_1(b,n)$ such that 
$$
(\frac{1}{b^2}-\eps)^n <\la_1(b,n) <(\frac{1}{b^2}+\eps)^n,
$$
and such that all the other eigenvalues are bigger than or equal to $(b-1)^2$. 
\end{lemma}
\begin{proof}
Let $K(b,n) = M(b,n) + \diag(b^2,0,0,\ldots,0)$, i.e.~we replace the anomalous $1$ on the diagonal with $b^2+1$. Let $\ka_1\le \ka_2\le\ldots\le \ka_n$ be the eigenvalues of $K(b,n)$ and let $\la_1\le \la_2\le \ldots \la_n$ be the eigenvalues of $M(b,n)$. Note that the norm of the matrix $K(b,n) - (b^2+1)\textrm I_m$ is $2b$, so we have the following claim.

\vspace{5pt}
\textbf{Claim A.} All the eigenvalues of $K(b,n)$ are larger or equal to $b^2+1-2b=(b-1)^2$.\qed
\vspace{5pt}

Let $D_n = \det(K(b,n))$ and $E_n = \det(M(b,n))$. By expanding both determinants along the final row we see that $D_n$ and $E_n$ fulfil the recurrence relations
$$
	D_{n+2} = (b^2+1)D_{n+1} - b^2 D_n\quad  	E_{n+2} = (b^2+1)E_{n+1} - b^2 E_n.
$$
Solving the recurrence in the standard way gives us $E_n=1$ for all $n$ and 
\beq\label{eq-det}
	D_n = \frac{b^2}{b^2-1} b^{2n} - \frac{1}{b^2-1}.
\eeq

\vspace{5pt}
\textbf{Claim B.} At least half of the eigenvalues of $K(b,n)$ are larger or equal to $b^2+1$.

\textit{Proof.} The claim follows from the fact that the matrix $\frac{1}{b}(K(b,n) - (b^2+1)\textrm I_m)$ is the adjacency matrix of a bipartite graph. The adjacency matrix of a bipartite graph has the property that its spectrum is symmetric around $0$, so there are exactly as many non-negative eigenvalues as there are non-positive eigenvalues. \qed
\vspace{5pt}

\textbf{Claim C.} The smallest eigenvalue $\la_1$ of $M(b,n)$ is smaller than $\frac{(b-1)^2}{2}$ for sufficiently large $n$. All the other eigenvalues of $M(b,n)$ are larger or equal to $(b-1)^2$.

\textit{Proof.} The Weyl inequality for rank $1$ perturbations (e.g.~\cite[Theorem 4.3.4]{MR1084815}) shows that the number of eigenvalues of $M(b,n)$ which are larger or equal to $b^2+1$ is at most one less than the number of eigenvalues of $K(b,n)$ which are larger or equal to $b^2+1$, so by Claim B we can crudely estimate it by $\frac{n}{3}$. It follows that the product  $\la_2\la_3\ldots \la_n$ is larger than $\frac{2}{(b-1)^2}$  when $n$ is sufficiently large. Since  $\la_1\la_2\ldots\la_n =E_n = 1$, we see that 
$$
\la_1 < \frac{(b-1)^2}{2}
$$
as claimed. The statement about the other eigenvalues of $M(b,n)$ follows again from the Weyl inequality and Claim A.\qed
\vspace{5pt}

We are ready to finish the proof now.  The statement about "all the other eigenvalues" is contained in Claim C.

It is easy to check that for every $k$ and $\eps$ there is $n_0$ such that for $n>n_0$  we have
$$
|\frac1n \tr K(b,n)^k - \frac1n \tr M(b,n)^k| <\eps.
$$
In other words,
$$
|\frac1n\sum_{i=1}^n \ka_i^k  - \frac1n\sum_{i=1}^n \la_i^k| <\eps.
$$

It follows, by the Weierstrass approximation of continuous functions by polynomials, that for every $\eps$  and a compactly supported continuous function $f$ defined on $\R$ there is $n_0$ such that for $n>n_0$ we have
$$
|\frac1n\sum_{i=1}^n f(\ka_i)  - \frac1n\sum_{i=1}^n f(\la_i)| <\eps.
$$
Let $f(x)$ be a compactly supported continuous function which is equal to $\ln(x)$ for $x\in [(b-1)^2, (b+1)^2]$ and which is $0$ for $x\le \frac{(b-1)^2}{2}$. Since $\frac1n\sum_{i=1}^n f(\ka_i)= \frac{1}{n} \sum_{i=1}^n \ln(\ka_i)$ and $\frac1n\sum_{i=1}^n f(\la_i) = \frac{1}{n}\sum_{i=2}^n \ln(\la_i)$ we get that for sufficiently large $n$ we have
$$
|\ln(D_n^{\frac{1}{n}}) - \ln((\la_2\ldots \la_n)^\frac{1}{n})| <\eps,
$$

From \eqref{eq-det} we see that $\ln(D_n^{\frac{1}{n}})$ converges to $\ln (b^2)$ when $n\to \infty$. It follows that $(\la_2\ldots \la_n)^\frac{1}{n}$ converges to $b^2$ with $n\to \infty$. Since $\la_1\la_2\ldots \la_n = E_n=1$ we see that $\la_1^{\frac1n}$ converges to $\frac{1}{b^2}$ as claimed.
\end{proof}

We introduce the following notation for the subsets of $\ZZ_2^\Z$. The elements of $\ZZ_2$ are denoted by $\0$ and $\1$. For 
 $\eps_i\in \{\0,\1\}$ we denote the set 
$$
	\{((m_i)\in \ZZ_2^\Z\colon m_{-a} = \eps_{-a}, \ldots, m_b = \eps_b,\}\subset \ZZ_2^\Z,
$$
by
$$
  [\eps_{-a}\eps_{-a+1}\ldots\eps_{-1}\underline{\eps_{0}}\eps_1\ldots\eps_b],
$$
and we let
$$
  \chi[\eps_{-a}\eps_{-a+1}\ldots\eps_{-1}\underline{\eps_{0}}\eps_1\ldots\eps_b, x] \in L^\infty(\ZZ_2^\Z)
$$ 
be the corresponding indicator function. Elements from the set above will be denoted with the curly brackets $()$ instead of $[]$.

For $b\in \R$ let $T(b)\in \ZZ \ltimes L^\infty(\ZZ_2^\ZZ)$ be defined as 
$$
T(b) := -b^2\chi[\1\u\0] + b(t[\u\0]+t^{-1}\chi[\0\u\ast]) +(b^2+1).
$$
In this notation, the operator studied in \cite{Grigorchuk_Zuk2001} was $t[\u\0]+t^{-1}\chi[\0\u\ast]$. Note that the indicator functions in the definition of $T(b)$ are in the image of the Pontryagin duality map $\Q[\oplus_\Z \ZZ_2]\into L^\infty(\ZZ_2^\Z)$. So, by Lemma \ref{lem-pontryagin}, the Novikov-Shubin invariant of $T(b)$ is the same as the Novikov-Shubin invariant of the corresponding $\wh{T(b)}\in \R[\ZZ \ltimes \oplus_\Z \ZZ_2 ]= \R[\ZZ_2\wr \ZZ]$.


\begin{theorem}
For $b>1$ the Novikov-Shubin invariant of $T(b)$ is equal to  $\frac1{2\log_{2} (b)}$.
\end{theorem}
\begin{proof}
We use Proposition \ref{prop-tool-free} with $X=  \ZZ_2^\Z$, $\Ga=\ZZ$, $A=\oplus_\Z \ZZ_2$. Let us compute two examples of a graph $\cal G(x)$.

First let $x= (\1\u \1)$. Then $x\notin [\1\u\0]$, $x\notin  [\u\0]$ and $x\notin [\0\u\ast]$, so the only outgoing arrow at $x$ is the self-loop  with label $(b^2+1)$. 

As for the incoming arrows at $x$, other than the self-loop, we see that $x\notin t.[\u\0]$ and $x\notin t^{-1}.[\0\u\ast]$, so there are no incoming arrows. Accordingly $\cal G(x)$ consists only of the vertex $x$ with a self-loop with label $b^2+1$.


Now let $x= (\1\u\0\0\1)$. Since $x\in  [\u\0]$ there is an outgoing arrow from $x$ to $t.x = (\1\0\u \0\1)$ with label $b$. Since $t.x\in [\u\0]$, there is an outgoing arrow from $t.x$ to $t^2.x = (\1\0\0\u\1)$ with label $b$. Since $t.x\in [\0\u\ast]$, there is also an outgoing arrow from $t.x$ to $x$ with label $b$. Similarly $t^2.x \in [\0\u\ast]$ so there is an arrow from $t^2.x$ to $t.x$ with label $b$.

As for the self-loops , $x\in [\1\u\0]$, so there is a self-loop at $x$ with label $(b^2+1)-b^2 = 1$. The vertices $t.x$ and $t^2.x$ have self-loops with labels $b^2+1$.

In analogy with these two examples we see that when $x\in [\1\u\0\0^k\1]$ then $\cal G(x)$ is the graph on Figure \ref{fig-app} with $k+2$ vertices.

\begin{figure}[here]
\centering
\begin{tikzpicture}
  [scale=1.1,auto=center]
  \tikzset{edge/.style = {->,> = latex'}}
  \node (n1) at (1,1) {$\bullet$};
  \node (n2) at (3,1)  {$\bullet$};
  \node (n3) at (5,1)  {$\ldots$};
  \node (n4) at (7,1) {$\bullet$};
  %\node (n5) at (9,1)  {};
  %\node (n6) at (11,1)  {6};

  \foreach \from/\to in {n1/n2,n2/n3,n3/n4}%,n3/n4,n4/n5,n5/n6}
    %\draw[edge] (\from) to (\to);
    %\draw[loop above,thick] (n1) to node {$1$} (n1);
    \draw[edge, bend right=23] (\from) to node[below] {$b$} (\to);% (n2) to[bend right=10] node[below] {$B\Rightarrow C$} (n3);
  \foreach \from/\to in {n1/n2,n2/n3,n3/n4}%,n3/n4,n4/n5,n5/n6}
    \draw[edge, bend right=23] (\to) to node[above] {$b$} (\from);
  \foreach \from/\to in {n2/n2,n4/n4}%,n3/n4,n4/n5,n5/n6}
    \draw[loop above,thick,edge] (\from) to node {$b^2+1$} (\to);
    \draw[loop above,thick,edge] (n1) to node {$1$} (n2);
\end{tikzpicture}
\caption{}\label{fig-app}
\end{figure}

 Let us check that, up to a set of measure $0$, every point of $X$ is in a connected component of $
 \cal G(x)$ for some $x\in [\1\u\0\0^k\1]$: 
$$
\mu ([\1\u \1]) + \sum_{k=0}^\infty (k+2)\mu([\1\u\0\0^k\1]) = \frac{1}{4} + \sum_{k=0}^\infty (k+2) \frac{1}{2^{k+3}} = \frac{1}{2}\sum_{k=1}^\infty \frac{k}{2^k} = 1.
$$
In particular the subset of those $x$ for which $\cal G(x)$ is finite is of full measure. Clearly the adjacency operator on the graph with $m$ vertices on Figure \ref{fig-app} is given by the matrix $M(b,m)$. Proposition \ref{prop-tool-free} now shows that 
$$
	\mu_T = \frac{1}{4} \mu_{\diag(b^2+1)} + \sum_{m=2} \frac{1}{2^{m+1}} \mu_{M(b,m)}.
$$

Let us use Lemma \ref{lem-matrix-lemma} to estimate $\mu_T((0,z])$ for small $z>0$. Let us fix a small $\eps$ in Lemma \ref{lem-matrix-lemma}. Then for sufficiently small $z$ we have
\beq\label{eq-sum}
\mu_T((0,z]) = \sum_{m\colon \la_1(b,m)\le z} \frac{1}{2^{m+1}}.
\eeq
By Lemma \ref{lem-matrix-lemma}, the smallest $m$ such that $\la_0(b,m)\le z$  is between
%~ 
%~ Let $n_0$ be the smallest natural number such that  $(\frac{1}{b^2}+\eps)^{n_0}\le z$, and let  $n_1$ be the smallest  such that $(\frac{1}{b^2}-\eps)^{n_1}\le z$. Clearly the first $m$ in the sum \eqref{eq-sum} lies between $m_0$
%~ 
%~ In other words 
%~ 
%~ and the smallest $m$ such that $\la_0(b,m)\le z$ is between the smallest 
%~ 
$$
\frac{|\log(z)|}{|\log(\frac{1}{b^2}+\eps)|}
$$
and 
$$
\frac{|\log(z)|}{|\log(\frac{1}{b^2}-\eps)|}.
$$

We estimate $\mu_T((0,z])$ from (i) below and (ii) above by taking in the sum \eqref{eq-sum} respectively (i) only the smallest $m$ such that $\la_1(b,m)\le z$, and (ii) the smallest such $m$ and all the natural numbers larger than $m$. We obtain that  $\mu_T((0,z])$ lies between
$$
2^{\frac{\log(z)}{|\log(\frac{1}{b^2}-\eps)|}} = z^\frac1{|\log(\frac{1}{b^2}-\eps)|}
$$
and
$$
2\cdot 2^{\frac{\log(z)}{|\log(\frac{1}{b^2}+\eps)|}} =2z^\frac1{|\log(\frac{1}{b^2}+\eps)|} 
$$
(in the algebraic manipulations we used that $\log(z)$ is negative for small $z$).

This shows that the Novikov-Shubin invariant of $T(b)$ lies between $\frac{1}{|\log(\frac{1}{b^2}-\eps)|}$ and  $\frac{1}{|\log(\frac{1}{b^2}+\eps)|}$, for every $\eps$, and so in fact must be equal to $\frac1{|\log(\frac{1}{b^2})|} = \frac{1}{2\log(b)}$. 
\end{proof}





%~ Consider the oriented graph $\wt{\cal G}$  whose set of vertices is $\Ga\times X$ and with an edge from $(\ga_1,x_1)$ to $(\ga_2,x_2)$  if for some instruction $(\ga_i,X_i)\in P$ we have $\ga_1.x\in X_i$ and $\ga_i\ga_1.x_1=\ga_2.x_2$. 
%~ 
%~ Let $\wt{\cal G}(x)$ be the connected component of $(e,x)$ in  $\wt{\cal G}$. Let $\wt{T}(x)\colon l^2(\wt{\cal G}(x)) \to l^2(\wt{\cal G}(x))$ be the adjacency operator on $\wt{\cal G}(x)$ and for $i=1,\ldots,n$ define $\wt\chi_i(x)\colon  l^2(\wt{\cal G}(x)) \to l^2(\wt{\cal G}(x)$ by $\wt\chi_i(x)\zeta_{(\ga,y)} := \zeta_{(\ga,y)}$ if $\ga.y\in X_i$ and $0$ otherwise. 
%~ 
%~ Consider the direct integral Hilbert space $\cal H := \int_X^\oplus l^2(\wt{\cal G}(x)) \, d\mu(x)$ (we will from now on suppress $\,d\mu(x)$ from the direct integral notation). 
%~ 
%~ The maps
%~ \beq\label{eq-iso}
    %~ T \mapsto \int^\oplus_{X} \wt T(x)\quad \chi_i \mapsto \int^\oplus_{X} \wt\chi_i(x)
%~ \eeq
%~ extend to a map $L (T,\chi_1,\ldots, \chi_n) \to B(\cal H)$, where $L (T,\chi_1,\ldots, \chi_n)$ is the von Neumann algebra generated by $T,\chi_1,\ldots, \chi_n$. . This map is a ${}^*$-isomorphism onto its image which sends the von Neumann trace on the left-hand side to the trace $\tau(\int^\oplus U(x)):= \int_X \langle \,U(x)\, \zeta_{(e,x)}, \zeta_{(e,x)}\rangle \,d\mu(x)$ on the right-hand side.







%~ 
%~ \section{The limit property}
%~ 
%~ We will now modify slightly the construction from the previous section to obtain group ring elements for which the limit property does not hold.
%~ 
%~ Let For $b,c\in \R$ let $T(b,c)\in \R[\ZZ_2\wr \ZZ]$ be defined as
%~ \begin{align}
%~ T(b,c) := &-b^2[\1\u\0\0] + b(t[\u\0\0]+t^{-1}[\0\u\0]) + (b^2+1)[\u\0] \\
%~ &-c^2[\0\u\1\1] +c(t[\u\1\1]+t^{-1}[\1\u\1]) + (c^2+1)[\u\1].
%~ \end{align}
%~ 
%~ \begin{theorem}
%~ Let $1<b<c$. Then $T(b,c)$ does not have the limit property. More precisely, for every $z_0>0$ there exists $z$ such that $0<z<z_0$ and 
%~ $$
%~ lala
%~ $$
%~ and there exists $z'$ such that  $0<z'<z_0$ and
%~ $$
%~ lolo
%~ $$
%~ \end{theorem}
%~ \begin{proof}
%~ 
%~ \end{proof}



%~ 
 %~ 
  %~ and define $\chi_i(x)\colon l^2(\cal G(x)) \to l^2(\cal G(x))$ by $\chi_i(x)\zeta_y := \zeta_y$ if $y\in X_i$ and $0$ otherwise. 
%~ 
%~ 
%~ 
%~ 
%~ \begin{proposition}
%~ Assume that $T$ defined above is sel
%~ \end{proposition}
%~ 
%~ 
%~ 
%~ and let $\wh S := 5+ 2(\wh T+\wh T^*) -4\wh\chi_I$.
%~ As explained in \cite[Section 2]{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem}, the spectral measure of $\wh S$ is the same as that of $S$.  In the next section, where we construct Turing dynamical systems which fulfils (A), (B) and (C), it can be checked directly that $\wh\chi_i$ are actually elements of $\Q[A]$ and so $\wh S\in \Q[A\rtimes \Ga]$.
%~ 
%~ 
%~ 
%~ 
%~ \begin{theorem}\label{thm-good-implies-main} Let $(X, T_X)$ be a Turing dynamical system as above which fulfils (A), (B) and (C). Consider the operator 
%~ $$
    %~ T:= \sum_{(\ga_i,X_i)\in P}  \ga_i \chi_i \in L^\infty(X) \rtimes \Ga , 
%~ $$
%~ where $P$ is the set of those instructions whose group element is not $e$. Let 
%~ $$
%~ S := 5+ 2(T+T^*) -4\chi_I\in L^\infty(X)\rtimes \Ga.
%~ $$
%~ Then there is a constant $C'>0$ and a sequence $\eps_j>0$ converging to $0$ such that 
%~ $$
%~ \mu((0,\eps_j)) \ge \frac{C'}{|\log(\eps_j)|^{d+1}}.
%~ $$
%~ \end{theorem}
%~ 
%~ The following statements, down to \eqref{eq-mu3} below, summarize \cite[Section 2]{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem}. In order to keep the discussion more straightforward, we translate the statements from \cite{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem} about groupoids to statements about graphs (this has the disadvantage that our notation is not compatible with the one from \cite{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem}).
%~ 
%~ Consider the oriented graph $\wt{\cal G}$  whose set of vertices is $\Ga\times X$ and with an edge from $(\ga_1,x_1)$ to $(\ga_2,x_2)$  if for some instruction $(\ga_i,X_i)\in P$ we have $\ga_1.x\in X_i$ and $\ga_i\ga_1.x_1=\ga_2.x_x$. 
%~ 
%~ Let $\wt{\cal G}(x)$ be the connected component of $(e,x)$ in  $\wt{\cal G}$. Let $\wt{T}(x)\colon l^2(\wt{\cal G}(x)) \to l^2(\wt{\cal G}(x))$ be the adjacency operator on $\wt{\cal G}(x)$ and for $i=1,\ldots,n$ define $\wt\chi_i(x)\colon  l^2(\wt{\cal G}(x)) \to l^2(\wt{\cal G}(x)$ by $\wt\chi_i(x)\zeta_{(\ga,y)} := \zeta_{(\ga,y)}$ if $\ga.y\in X_i$ and $0$ otherwise. 
%~ 
%~ Consider the direct integral Hilbert space $\cal H := \int_X^\oplus l^2(\wt{\cal G}(x)) \, d\mu(x)$ (we will from now on suppress $\,d\mu(x)$ from the direct integral notation). 
%~ 
%~ The maps
%~ \beq\label{eq-iso}
    %~ T \mapsto \int^\oplus_{X} \wt T(x)\quad \chi_i \mapsto \int^\oplus_{X} \wt\chi_i(x)
%~ \eeq
%~ extend to a map $L (T,\chi_1,\ldots, \chi_n) \to B(\cal H)$, where $L (T,\chi_1,\ldots, \chi_n)$ is the von Neumann algebra generated by $T,\chi_1,\ldots, \chi_n$. . This map is a ${}^*$-isomorphism onto its image which sends the von Neumann trace on the left-hand side to the trace $\tau(\int^\oplus U(x)):= \int_X \langle \,U(x)\, \zeta_{(e,x)}, \zeta_{(e,x)}\rangle \,d\mu(x)$ on the right-hand side.
%~ 
%~ Consider the oriented edge-labelled graph $\cal G$ whose set of vertices is $X$, with an edge labelled $\ga_i$ from $x_1$ to $x_2$ if $(\ga_i,X_i)\in P$, $x_1\in X_i$ and $\ga_i.x_1=x_2$. Let $\cal G(x)$ be the connected component of $x$. Let $T(x) \colon l^2(\cal G(x)) \to l^2(\cal G(x))$ be the adjacency operator on $\cal G(x)$ and define $\chi_i(x)\colon l^2(\cal G(x)) \to l^2(\cal G(x))$ by $\chi_i(x)\zeta_y := \zeta_y$ if $y\in X_i$ and $0$ otherwise. 
%~ 
%~ We say $\cal G(x)$ is \textit{simply-connected} if multiplying edge-labels along any closed loop gives the trivial element of $\Ga$ (if a loop traverses an edge in the direction opposite to the orientation of the edge, we invert the label). Let $X^s$ be the subset of $X$ consisting of all points whose connected components are simply-connected.
%~ 
%~ 
%~ 
%~ It is clear that if $\cal G(x)$ is simply-connected then the natural map $\wt{\cal G}(x) \to \cal G(x)$ is a graph isomorphism which intertwines $\wt T(x)$ with $\wt T$ and $\wt \chi_i$ with $\chi_i$. It follows  that the map $L (T,\chi_1,\ldots, \chi_n) \to B(\int^\oplus l^2(\wt{\cal G}(x)) \oplus \int^\oplus l^2(\cal G(x)))$ given by \beq\label{eq-iso2}
    %~ U \mapsto \int^\oplus_{X\setminus X^s} \wt U(x) \oplus \int^\oplus_{X^s} U(x) %\quad \chi_i \mapsto \int^\oplus_{X\setminus X^s}\wt\chi_i(x) \oplus \int^\oplus_{X^s} \chi_i(x)
%~ \eeq
%~ also 
%~ %extend to a map $L (T,\chi_1,\ldots, \chi_n) \to B(\int^\oplus l^2(\wt{\cal G}(x)) \oplus \int^\oplus l^2(\cal G(x)))$ which 
%~ is a ${}^*$-isomorphism onto its image, and it sends the von Neumann trace on the left-hand side to the trace 
%~ \begin{multline*}
%~ \tau\left(\int^\oplus_{X\setminus X^s} U(x) \oplus \int^\oplus_{X^s} U(x) \right):= \\=\int_{X\setminus X^s} \langle \,U(x)\, \zeta_{(e,x)}, \zeta_{(e,x)}\rangle \,d\mu(x) + \int_{X^s} \langle \,U(x)\, \zeta_{x}, \zeta_{x}\rangle \,d\mu(x)
%~ \end{multline*}
%~ 
%~ Finally, let $X^{sf}$ be the subset of $X^s$ consisting of points whose connected component in $\cal G$ is finite. We can write the map \eqref{eq-iso2} as 
%~ \beq\label{eq-iso3}
       %~ U \mapsto \int_{X\setminus X^s}^\oplus \wt U(x) \oplus \int_{X^s\setminus X^{sf}}^\oplus U(x)\oplus \int_{X^{sf}}^\oplus U(x),
%~ \eeq
%~ A simple computation shows that
%~ \beq\label{eq-tr}
%~ \int_{X^{sf}}\langle \,U(x)\, \zeta_{x}, \zeta_{x}\rangle \,d\mu(x) = \int_{X^{sf}} \frac{1}{|\cal G(x)|} \tr(T(x))\,d\mu(x),
%~ \eeq
%~ where $\tr(T(x)) = \sum_{v\in G(x)} \langle T(x)\zeta_v,\zeta_v\rangle\,d\mu(x) $ is the standard trace of a finite-dimensional endomorphism.
%~ 
%~ It is not difficult to sea, that on the right-hand side on the integral over $X^{sf}$ we can take the trace to be $\tau(\cdot) := \int_{X^{sf}} \frac{1}{|\cal G(x)|} \tr(T(x))$, where $\tr(T(x)) = \sum_{v\in G(x)} \langle T(x)\zeta_v,\zeta_v\rangle\,d\mu(x) $ is the standard trace.
%~ 
%~ Since the map \eqref{eq-iso3} is a trace-preserving isomorphism, and $S\in L (T,\chi_1,\ldots, \chi_n)$, the spectral measure $\mu_S$ decomposes into the sum $\mu_1+\mu_2+\mu_3$ corresponding to the three direct summands. We will show that already $\mu_3$ fulfils the claimed inequality. 
%~ 
%~ Equation \eqref{eq-tr} implies that $\mu_3$ is an integral of spectral measures of \textit{finite-dimensional} adjacency operators $S(x), x\in X^{sf}$:
%~ \beq\label{eq-mu3}
%~ \mu_3 = \int_{X^{sf}} \frac{1}{|\cal G(x)|}\mu_{S(x)} \, d\mu(x),
%~ \eeq
 %~ so it is relatively easy to compute.



==> coaster-operator.tex <==
\section{Computational tool in the case of a non-free action}\label{sec-tool-non-basic}

We will now repeat the discussion from Section \ref{sec-tool-basic}, and add some extra structure in order to deal with a non-free action. For the proofs see  \cite[Section 2]{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem}.

Let $\Ga\actson X$ be as in Section \ref{sec-tool-basic}, with the exception that it is not necessarily a free action. Let $T\in \Ga\ltimes L^\infty(X)$ be defined as $T := \sum_{i=1}^n a_i\ga_i\chi_i$ (with the notation from Section \ref{sec-tool-basic}).

Consider the oriented graph $\cal G_\Ga$ whose set of vertices is $X$, and with edges labelled by the elements of the set  $\{\ga_1,\ldots,\ga_n\}$, defined as follows. There is an edge with label $\ga_i$ from $x_1$ to $x_2$ if $x_1\in X_i$ and $\ga_i.x_1=x_2$. Let $\cal G_\Ga(x)$ be the connected component of $x$.  We say $\cal G_\Ga(x)$ is \textit{simply-connected} if multiplying edge-labels along any closed loop gives the trivial element of $\Ga$ (if a loop traverses an edge in the direction opposite to the orientation of the edge, we invert the label). 

Let $\cal G(x)$ be the graph which arises from $\cal G_\Ga(x)$ by changing the  label $\ga_i$ on the edge between $x_1$ and $x_2$ as above to the sum
$$
	\sum_{\mathclap{\substack{j\colon \ga_j=\ga_i\\x_1\in X_j}}} a_j.
$$
Finally let  $T(x) \colon l^2(\cal G(x)) \to l^2(\cal G(x))$ be the adjacency operator on $\cal G(x)$.

%Let $X^s$ be the subset of $X$ consisting of all points whose connected components are simply-connected.

\begin{proposition}\label{prop-tool-non-free}
Let us assume that the set of $x$ such that  $\cal G_\Ga(x)$ is finite and simply-connected  is of full measure. Then $\dimvn\ker T$ is equal to 
$$
\int_X \frac{\dim\ker{T(x)}}{|\cal G(x)|}\,d\mu(x).
$$\qed
\end{proposition}

\section{Irrational $l^2$-Betti numbers arising from $\ZZ_p\wr \ZZ$}\label{sec-the-operator}

For the rest of the article let $X$ be the compact abelian group $\ZZ_p^\Z\times \ZZ_2^3$, and $\Ga = \ZZ \times \aut(\ZZ_2^3)$. The action $\Ga {\actson} X$ is the natural one, i.e.~$\aut(\ZZ_2^3)$ acts on $\ZZ_2^3$ and $\ZZ$ acts on $\ZZ_p^\Z$ by shifting the coordinates.

Note that  $\Ga\ltimes A $ is isomorphic to $\ZZ_p \wr \ZZ \times (\aut(\ZZ_2^3)\ltimes \ZZ_2^)$. We will shortly define $T \in \Q[\Ga\ltimes A]$ such that 
$$
\dimvn\ker T = \frac{4p^3+3p^2+2p-1}{8p^3} + \frac1{8p^2(p-1)} \sum_{k=1}^\infty (\frac{p-1}{p})^{k+2^{k-1}},
$$

The additional factor $1344$ in Theorem \ref{thm-intro-zero} comes from the fact that $\ZZ_p\wr\ZZ$ is a  subgroup in $\Ga\ltimes A$ of index $1344$ (see e.g.~\cite[Lemma 6.2]{grabowski-on-turing-dynamical-systems-and-the-atiyah-problem} for more explanation). Furthermore, for $k\neq 0$ the kernels of $T$ and $kT$ are the same, so we will also obtain a matrix over $\Z[\Ga\ltimes A]$ whose kernel dimension is as above.


Let $A$, $B$, $C$, $D$, $F$, $I$, $U_1$, $U_2$ ($U$ stands for \textit{unimportant}, $F$ for \textit{final} and $I$ for \textit{initial}) denote the elements of $\Zmod{2}^3$. The only assumption on this labelling is  that the first $6$ symbols correspond to non-zero elements of $\Zmod{2}^3$.

For every pair $(x,y)$ of different elements from the set $\{A, B, C,D, F, I\}$ we fix an automorphism denoted  by $(x\to y)\in \aut(\Zmod{2}^3)$ which sends
$x$ to $y$, in such a way that  
\begin{equation}\label{eq_loops_inv}
(x\to y) = (y\to x)^{-1}
\end{equation}
and
\begin{equation}\label{eq_loops_init}
(C\to D)(A\to C)=(I\to D)(A\to I).
\end{equation}
To treat the case of an arbitrary $p$, we change our notation in the following way. 
Let $\0 := \{0\} \subset \ZZ_p$ and $\1 := \{1,2,3,\ldots, p-1\}\subset \ZZ_p$. Let
$$
  [\eps_{-a}\eps_{-a+1}\ldots\eps_{-1}\underline{\eps_{0}}\eps_1\ldots\eps_b, x],
$$
where $\eps_i\in \{\0,\1\}$, denote  
$$
	\{((m_i), y)\in \Zmod{p}^\Z \times \Zmod{2}^3: m_{-a} \in \eps_{-a}, \ldots, m_b \in \eps_b, y= x\}\subset X,
$$
and let  
$$
  \chi[\eps_{-a}\eps_{-a+1}\ldots\eps_{-1}\underline{\eps_{0}}\eps_1\ldots\eps_b, x] \in L^\infty(X)
$$ 
be the corresponding indicator function.

Let $S \in \Q[\Ga\ltimes A]$ be represented by the sum of the following terms:
\begin{align}
 \label{eq_Sdef_1} ( -t(I\to D) + t^{-1}(I\to A)) &\cdot \chi[\1\underline{\0}\1,I]		\\
  (-t^2(A\to C) - 2t^{-1} ) &\cdot\chi[\1\underline{\1}\0\1,A]	\nonumber		\\
 -t^2(A\to C)		&\cdot	\chi[\0\underline{\1}\0\1,A]\nonumber	\\
 -2t^{-1} &\cdot\chi [\1\underline{\1}\0\0,A]			\nonumber	\\
 0 &\cdot \chi[\0\underline{\1}\0\0,A]				\nonumber\\
  -2t^{-1} &\cdot \chi[\1\underline{\1}\1,A]				\nonumber\\
 -(A\to B) &\cdot \chi[\0\underline{\1}\1,A]			\nonumber	\\
  -t  &\cdot \chi[\underline{\1}\1,B]		\nonumber		\\
  -(B\to A) &\cdot \chi[\underline{\1}\0,B]		\nonumber		\\
  (-t + (C\to D)) &\cdot \chi[\underline{\1}\1,C]	\nonumber			\\
 +(C\to D)  &\cdot \chi[\underline{\1}\0,C]		\nonumber		\\
 -t   &\cdot \chi[\underline{\1}\1,D]		\nonumber		\\
  -(D\to F) &\cdot \chi[\underline{\1}\0,D]		\nonumber		\\
 0	&\cdot \chi[\underline{\1}\0,F]		\nonumber		\\
 0 		&\cdot \chi_U,					\nonumber
\end{align}
where $e$ is the neutral element and  $\chi_U$ is the indicator function of the set $U$ defined to be  ``all the rest'', i.e.~the union of the sets $[\1\underline{\0}\1,I]$,
$[\1\underline{\1}\0\1,A]$, $[\0\underline{\1}\0\1,A]$, $[\1\underline{\1}\0\0,A]$, $[\0\underline{\1}\0\0,A]$,
$[\1\underline{\1}\1,A]$, $[\0\underline{\1}\1,A]$, $[\underline{\1}\1,B]$, $[\underline{\1}\0,B]$, $[\underline{\1}\1,C]$.
$[\underline{\1}\0,C]$, $[\underline{\1}\1,D]$,  $[\underline{\1}\0,D]$ and $[\underline{\1}\0,F]$. 

Finally define
\begin{equation}\label{eq_Tdef}
	T:=S + 1-\chi_U - \chi[\1\underline{\0}\1,I] - \chi[\underline{\1}\0,F]
\end{equation}

\begin{remark}\label{rem-it-is-easy}
The reason we explicitly write the  terms "$0\scdot \ldots$" is that this way the right hand sides are indicator functions of disjoint sets whose union is $X$. This is helpful when checking that the connected components $\cal G_\Ga(x)$ are as claimed. To reassure the reader, without any $0$-terms it would be the same operator and the same computations would have to be performed.
\end{remark}

We will now describe the  graphs $\cal G_\Ga(x)$  and $\cal G(x)$ for  $x\in X$. It is convenient to describe them in four families, which we do in separate subsections. 

We will show figures for the graphs, but for clarity we suppress self-loops. Note that the self-loops are given only by the terms in  \eqref{eq_Tdef}, so it is also easy to take them into account.

In all the cases it is somewhat tedious but, using Remark \ref{rem-it-is-easy},  straightforward to check that the graph $\cal G_\Ga(x)$ is as claimed for a given $x\in X$.

\subsection{Case 1: $x\in U$}\label{subsec_sgraph_u}\mbox{}

The graph $\cal G_\Ga(x)$ consists of just one vertex with no edges. Accordingly, the adjacency operator $T(x)$ is the $0$ operator. We clearly deduce the following lemma.

%\begin{figure}[h]%
  %\resizebox{0.029\textwidth}{!}{\input{sgraph-u.pdf_t}}
  %\caption{$\cal R(\UU, T)$}
  %\label{fig_sgraph_u}
%\end{figure}

\begin{lemma}We have the following properties.\label{lemma_sgraph_u}
\mbox{}
\begin{enumerate}
 \item $\dim\ker T(x)  = 1$.
% \item The $S$-graph $\mathbf u$ does not possess non-trivial automorphisms.
 \item $\cal G_\Ga(x)$ is simply-connected. 
 \item $\mu (U) =\frac{1}{8}(2+5\frac1p+ \frac{1}{p^{3}} + 2\frac{p-1}{p^3} + \frac{p-1}{p} + (\frac{p-1}{p})^2) $
\end{enumerate}
\end{lemma}
\begin{proof}
(1) and (2) are clear. As for (3), note that we can explicitly write
\begin{align*}
U &= [\underline{\0}, A] \sqcup [\underline{\0}, B] \sqcup [\underline{\0},C] \sqcup [\underline{\0}, D] \sqcup [\cdot, U_1] \sqcup [\cdot, U_2] \sqcup\\ & \sqcup [\underline{\0}, F] \sqcup [\underline{\1}\1, F] \sqcup [\underline{\1}, I] \sqcup
[\1\underline{\0}\0, I] +\sqcup [\0\underline{\0}\1, I] \sqcup [\0\underline{\0}\0,I].
\end{align*}
Since $\mu$ is the product measure, it is easy to compute the measures of the sets above. We start with  $\mu([\u\0]) = \frac{1}{p}$, $\mu([\u\1]) = \frac{p-1}{p}$, and then for example $\mu([\0\uz\1, I]) = (\frac{1}{p})^2\scdot \frac{p-1}{p}\scdot \frac{1}{8}$.
\end{proof}



\subsection{Case 2: $x\in [\0\uo\1^{k-1}\0\0,A]$}\label{subsec_sgraph_g}\mbox{} 

If we denote $x =(\0\uo\1^{k-1}\0\0,A)$, then the vertices of $\cal G_\Ga(x)$ are  
\begin{align*}
(\0\uo\1^{k-1}\0\0,A)\quad (\0\1\uo\1^{k-2}\0\0,A)\quad \ldots,\quad (\0\1^{k-1}\uo\0\0,A) \\
(\0\uo\1^{k-1}\0\0,B) \quad (\0\1\uo\1^{k-2}\0\0,B)\quad \ldots\quad (\0\1^{k-1}\uo\0\0,B).
\end{align*}

$\cal G_\Ga(x)$ is shown on Figure \ref{fig_sgraph_g_emb}. Each vertex should additionally have a self-loop with label $e$. To avoid clutter only some vertices are explicitly identified as elements of $X$.

To facilitate to the reader checking that $\cal G_\Ga(x)$ is as claimed we indicate that the corresponding terms in \eqref{eq_Sdef_1}  are
\begin{align*}
[\0\uo\1,A]& \quad[\1\uo\1,A]&\quad\ldots&\quad [\1\uo\1,A]&\quad[\1\uo\0\0, A]& \\
[\uo\1,B]& \quad[\uo\1,B]&\quad\ldots&\quad [\uo\1,B]&\quad[\uo\0, B]&.
\end{align*}

The graphs $\cal G (x)$ are shown  on Figure \ref{fig_sgraph_g}. Each vertex should additionally have a self-loop with label $1$. 

\begin{figure}[h]%
  \resizebox{0.8\textwidth}{!}{\input{sgraph-g-emb.pdf_t}}
  \caption{$\cal G_\Ga(x)$ without self-loops for $x= (\0\uo\1^{k-1}\0\0,A)$.}
  \label{fig_sgraph_g_emb}
\end{figure}

\begin{figure}[h]%
  \resizebox{0.84\textwidth}{!}{\input{sgraph-g.pdf_t}}
  \caption{$\cal G(x)$ without self-loops for $x= (\0\uo\0\0,A)$, $x= (\0\uo\1\0\0,A)$, and $x= (\0\uo\1^{k-1}\0\0,A)$.}
  \label{fig_sgraph_g}
\end{figure}

\begin{lemma}\label{lemma_sgraph_g}We have the following properties.
\begin{enumerate}
 \item $\dim \ker T(x) = 0$
 \item $\cal G_\Ga(x)$ is simply-connected. 
 \item \textsc{$\mu ( [\0\uo\1^{k-1}\0\0,A]) = \frac18\cdot (\frac{1}{p})^3\cdot (\frac{p-1}{p})^k$} and $|\cal G(x)| = 2k$.
\end{enumerate}
\end{lemma}
\begin{proof}
(2) follows easily from Figure \ref{fig_sgraph_g_emb} and Equation \eqref{eq_loops_inv}. (3) is a direct computation as in Lemma \ref{lemma_sgraph_u}. (1) follows from analysing Figure \ref{fig_sgraph_g}, but for completeness we give a proof in the appendix.
\end{proof}

\subsection{Case 3: $x\in [\0\0\uo\1^{l-1}\0,C]$}\label{subsec_sgraph_h}\mbox{}

If we denote $x =(\0\0\uo\1^{l-1}\0,C)$ then the vertices of $\cal G_\Ga(x)$ are 	
\begin{align*}
(\0\0\uo\1^{l-1}\0,C)&\quad  \ldots&\quad (\0\0 \1^{l-1}\uo\0,C)& \\
(\0\0\uo\1^{l-1}\0,D)& \quad \ldots& \quad (\0\0 \1^{l-1}\uo\0,D)& \\
&&(\0\0 \1^{l-1}\uo\0,F)&
\end{align*}

$\cal G_\Ga(x)$ is shown on Figure \ref{fig_sgraph_h_emb}. Each vertex except the final one should additionally have a self-loop with label $e$. To avoid clutter only some vertices are explicitly identified as elements of $X$.

To facilitate to the reader checking that $\cal G_\Ga(x)$ is as claimed we indicate that the corresponding terms in \eqref{eq_Sdef_1}  are
\begin{align*}
[\uo\1,C],\quad \ldots,\quad [\uo\1,C],\quad [\uo \0,C], \\
[\uo\1,D], \quad\ldots, \quad [\uo\1,D], \quad[\uo \0,D], \\
[\uo \0, F].
\end{align*}

The graphs $\cal G (x)$ are shown  on Figure \ref{fig_sgraph_h}.  Each vertex except the final one should additionally have a self-loop with label $1$. 

\begin{figure}[h]%
  \resizebox{0.62\textwidth}{!}{\input{sgraph-h-emb.pdf_t}}
  \caption{$\cal G_\Ga(x)$ without self-loops for $x= (\0\0\,\uo\1^{l-1}\0,C)$.}
  \label{fig_sgraph_h_emb}
\end{figure}


\begin{figure}[h]%
  \resizebox{0.74\textwidth}{!}{\input{sgraph-h.pdf_t}}
  \caption{$\cal G(x)$ without self-loops for $x= (\0\0\,\uo\0,C)$, $x= (\0\0\,\uo\1\0,C)$, and $x= (\0\0\,\uo\1^{l-1}\0,C)$}
  \label{fig_sgraph_h}
\end{figure}


\begin{lemma} The following properties are true.\label{lemma_sgraph_h}\begin{enumerate}
 \item $\dim \ker T(x) = 1$
 \item $\cal G_\Ga(x)$ is simply-connected. 
 \item \textsc{$\mu ( [\0\0\uo\1^{l-1}\0,C]) = \frac18\cdot (\frac{1}{p})^3 \cdot (\frac{p-1}{p})^l$} and $|\cal G(x)| = 2l+1$.
\end{enumerate}
\end{lemma}
\begin{proof}
(2) follows easily from Figure \ref{fig_sgraph_h_emb} and Equation \eqref{eq_loops_inv}. (3) is a direct computation as in Lemma \ref{lemma_sgraph_u}. (1) follows from analysing Figure \ref{fig_sgraph_h}, but for completeness we give a proof in the appendix.
\end{proof}


\subsection{Case 4: $x\in [\0\uo\1^{k-1}\0\1^l\0,A]$}\label{subsec_sgraph_j} \mbox{}

If we denote $x=(\0\uo\1^{k-1}\0\1^l\0,A)$ then the vertices of $\cal G_\Ga(x)$ are 
\begin{align*}
(\0\uo\1^{k-1}\0\1^l\0,A),\,\,  (\0\1\uo\1^{k-2}\0\1^l\0,A),\,\,  \ldots,\,\, (\0\1^{k-1}\uo\0\1^l\0,A), \\
(\0\uo\1^{k-1}\0\1^l\0,B),\,\,  (\0\1\uo\1^{k-2}\0\1^l\0,B), \,\, \ldots,\,\,  (\0\1^{k-1}\uo\0\1^l\0,B),\\
(\0\1^{k}\uz\1^l\0,I),\\
(\0\1^k\0\uo\1^{l-1}\0,C), \,\, \ldots,\,\,  (\0\1^k\0 \1^{l-1}\uo\0,C), \\
(\0\1^k\0\uo\1^{l-1}\0,D), \,\, \ldots,\,\,  (\0\1^k\0 \1^{l-1}\uo\0,D), \\
(\0\1^k\0 \1^{l-1}\uo\0,F).
\end{align*}

$\cal G_\Ga(x)$ is shown  on Figure  \ref{fig_sgraph_j_emb}. Each vertex except the final and the initial ones should additionally have a self-loop with label $e$. To avoid clutter only some vertices are explicitly identified as elements of $X$. Because it could be unclear which labels correspond to which vertices, the identified vertices are marked white. 

To facilitate to the reader checking that $\cal G_\Ga(x)$ is as claimed we indicate that the corresponding terms in \eqref{eq_Sdef_1}  are
\begin{align*}
[\0\uo\1,A],\quad[\1\uo\1,A],\quad\ldots,\quad[\1\uo\1,A],\quad[\1\uo\1\0\1, A], \\
[\uo\1,B],\quad[\uo\1,B],\quad\ldots,\quad[\uo\1,B],\quad[\uo\0, B],\\
[\1\underline{\0}\1, I],\\
[\uo\1,C],\quad \ldots, \quad[\uo\1,C], \quad[\uo \0,C], \\
[\uo\1,D], \quad\ldots, \quad[\uo\1,D],\quad [\uo \0,D], \\
[\uo \0, F].
\end{align*}

The graphs $\cal G (x)$ are shown  on Figure \ref{fig_sgraph_j}.  Each vertex except the final and the initial ones should additionally have a self-loop with label $1$.
 
\begin{figure}[h]%
  \resizebox{0.87\textwidth}{!}{\input{sgraph-j-emb.pdf_t}}
  \caption{$\cal G_\Ga(x)$ without self-loops for $x= (\0\uo\1^{k-1}\0\1^l\0,A)$.}  \label{fig_sgraph_j_emb}
\end{figure}

\begin{figure}[h]%
  \resizebox{0.95\textwidth}{!}{\input{sgraph-j.pdf_t}}
  \caption{$\cal G(x)$ without self-loops for $x= (\0\uo\1^{k-1}\0\1^l\0,A)$}
  \label{fig_sgraph_j}
\end{figure}


\begin{lemma}The following properties are true.\label{lemma_sgraph_j}
\begin{enumerate}
 \item $\dim \ker T(x) = \left\{ 
	\begin{array}{l l}
  		2 & \quad \mbox{if $l=2^{k-1}-1$ }\\
		1 & \quad \mbox{otherwise}\\ 
	\end{array} \right. $
 \item $\cal G_\Ga(x)$ is simply-connected. 
 \item \textsc{$\mu ([\0\uo\1^{k-1}\0\1^l\0,A]) = \frac18\cdot (\frac{1}{p})^3\cdot (\frac{p-1}{p})^{k+l}$} and $|\cal G(x)| = 2k+2l+2$.
\end{enumerate}
\end{lemma}
\begin{proof}
(2) follows easily from Figure \ref{fig_sgraph_j_emb} and Equations \eqref{eq_loops_inv} and \eqref{eq_loops_init}. (3) is a direct computation as in Lemma \ref{lemma_sgraph_u}. (1) follows from analysing Figure \ref{fig_sgraph_h}, but for completeness we give a proof in the appendix.
\end{proof}

\subsection{Checking that we have not missed any graphs}\mbox{}

We need to check that the graphs $\cal G(x)$ on Figures \ref{fig_sgraph_g_emb}, \ref{fig_sgraph_h_emb} and \ref{fig_sgraph_j_emb}, together with the set $U$ cover the whole space $X$. To this end we compute that the measure of the covered part is $1$, by using the formulas in Lemmas \ref{lemma_sgraph_u}(3), \ref{lemma_sgraph_g}(3), \ref{lemma_sgraph_h}(3) and \ref{lemma_sgraph_j}(3).

Let $\al :=\frac{1}{p}$, $\be := \frac{p-1}{p}$. We need to check that  
\begin{multline*}
\frac{1}{8}(2+5\al+ \al^3 + 2\be\al^2 + \be + \be^2) \,\,+\,\,
\sum_{k=1}^\infty 2k\scdot \frac18\scdot \al^3\scdot \be^k \,\,+\,\,\\
+\sum_{l=1}^\infty (2l+1)\scdot \frac18\scdot \al^3 \scdot \be^l \,\,+\,\,
\sum_{k,l=1}^\infty (2k+2l+2) \scdot \frac18\scdot \al^3\scdot \be^{k+l} \,=\,1.
\end{multline*}

This is a tedious but elementary exercise in using the formula 
$$
	\sum_{n=1}^\infty (n+C) x^n = \frac{x}{(1-x)^2} + \frac{Cx}{1-x},
$$
valid for $0\le x \le 1$.
%~ 
%~ By now we check that the measure of the set of points know that $\UU$, $\GG(k)$, $\HH(l)$ and $\JJ(k,l)$ form a family of disjoint good basic graphs for $T$. We proceed to check that they are an exhausting family, i.e. that they fulfill the equation \eqref{eq:exhausting-graph-sequence}.  From the previous subsections we know that
%~ \begin{align*}
 %~ &\mu (\supp (\UU))) =\frac{1}{8}(2+5\al+ \al^3 + 2\be\al^2 + \be + \be^2), \\
 %~ &\mu (\supp (\GG(k))) = 2k\cdot \frac18\cdot \al^3\cdot \be^k,\\
 %~ &\mu (\supp (\HH(l))) = (2l+1)\cdot \frac18\cdot \al^3 \cdot \be^l,\\
 %~ &\mu (\supp (\JJ(k,l))) =(2k+2l+2) \cdot \frac18\cdot \al^3\cdot \be^{k+l},
%~ \end{align*} 
%~ 
%~ We will freely use that $\al+\be =1$. Recall the formula
%~ $$
	%~ \sum_{n=1}^\infty (n+C) x^n = \frac{x}{(1-x)^2} + \frac{Cx}{1-x}
%~ $$
%~ for $0\le x \le 1$. Using it we see that 
%~ $$
%~ \sum_{k\ge 1} 2k\cdot \frac18\cdot \al^3\cdot
%~ \be^k= \frac{\al^3}{4} \sum_{k\ge 1} k \be^k = \frac{\al^3}{4}\cdot \frac{\be}{\al^2}=\frac{\al \be}{4}.
%~ $$ 
%~ Similarly 
%~ $$\sum_{l\ge 1} (2l+1)\cdot \frac18\cdot \al^3 \be^l =
%~ \frac{\al^3}{4}\sum_{l\ge 1} l \be^l  + \frac{\al^3}{8}\sum_{l\ge 1} \be^l = 
%~ \frac{\al\be}{4} + \frac{\al^3}{8} \frac{\be}{1-\be} =
%~ \frac{\al\be}{4} + \frac{\al^2\be}{8}.
%~ $$
%~ Finally
%~ \begin{eqnarray*}
%~ \sum_{k,l\ge 1} (2k+2l+2)\cdot \frac18\cdot \al^3 \be^{k+l} &=& \frac{\al^3}{4} \sum_k \be^k\sum_l
%~ (l+ (k+1))\be^l 
%~ \,\,= \,\,\frac{\al^3}{4} \sum_k \be^k(\frac{(k+1)\be}{\al}+ \frac{\be}{\al^2}) \\
%~ &=&\frac{\al^2\be}{4} \sum_k (k+1)\be^k + \frac{\al\be}{4} \sum_k \be^k  
%~ \,\,=\,\, \frac{\al^2\be}{4}(\frac{\be}{\al^2} + \frac{\be}{\al}) + \frac{\al\be}{4} \frac{\be}{\al} \\
%~ &= &\frac{\be^2}{2} +\frac{\al\be^2}{4}.
%~ \end{eqnarray*}
%~ Putting everything together, we get 
%~ \begin{multline*}
%~ \frac{1}{8}(2+5\al+ \al^3 + 2\be\al^2 + \be + \be^2) \,+\,
%~ \frac{\al \be}{4} \,+\, 
%~ (\frac{\al\be}{4} + \frac{\al^2\be}{8}) \,+\,
%~ (\frac{\be^2}{2} +\frac{\al\be^2}{4}) \,=\, \\
%~ \,=\,  
%~ \left(\frac14 +\frac58\al + \frac18\al^3 + \frac14\al^2 - \frac14\al^3 + \frac18 -\frac18\al
%~ +\frac18-\frac14\al+\frac18\al^2\right) \,+\, \\
%~ \,+\, \left( \frac14\al - \frac14\al^2\right) + \left(\frac14\al - \frac14\al^2 +\frac18\al^2
%~ -\frac18\al^3\right)  + \left(\frac12 -\al+\frac12\al^2 + \frac14\al-\frac12\al^2+\frac14\al^3\right) \,=\,
 %~ 1,
%~ \end{multline*}
%~ as required.

\subsection{The end game}\label{subsec-the-end-game}\mbox{}

We are now in a position to use Proposition \ref{prop-tool-non-free}. The following corollary, together with the discussion at the beginning of Section \ref{sec-the-operator}, proves Theorem \ref{thm-intro-zero}.

\begin{cory}\label{cory_dimT} We have
$$
\dimvn\ker T =
\frac{4p^3+3p^2+2p-1}{8p^3} + \frac1{8p^3} \sum_{k=1}^\infty (\frac{p-1}{p})^{k+2^{k}},
$$ which is a transcendental number.
\end{cory}
\begin{proof}

Let $T_0$ be the $0$ operator $\C\to \C$, let $T_1(k)\colon \C^{2k}\to\C^{2k}$ be the adjacency operator on the graph from Figure \ref{fig_sgraph_g}, let $T_2(l)\colon \C^{2l+1}\to \C^{2l+1}$ be the adjacency operator on the graph from Figure \ref{fig_sgraph_h}, and finally let $T_3(k,l)\colon \C^{2k+2l+2} \to \C^{2k+2l+2}$ be the adjacency operator on the graph from Figure \ref{fig_sgraph_j}.

By Proposition \ref{prop-tool-non-free} and the computations in the previous subsections, the left-hand side is equal to the sum of the following terms
\begin{gather*}
 	\frac{1}{8}(2+5\al+ \al^3 + 2\be\al^2 + \be + \be^2) \cdot \dim\ker T_0, \\
 	\sum_{k=1}^\infty \frac18\cdot \al^3\cdot \be^k\cdot \dim\ker T_1(k), \\
 	\sum_{l=1}^\infty \frac18\cdot \al^3 \be^l \dim\ker T_2(l),  \\
 	\sum_{k,l=1}^\infty \frac18\cdot \al^3 \be^{k+l} \dim\ker T_3(k,l).
\end{gather*}
Substituting the values for the kernel dimensions we get
\begin{multline*}
	\frac{1}{8}(2+5\al+ \al^3 + 2\be\al^2 + \be + \be^2) \,+\,0 \,+\, \sum_{l=1}^\infty \frac18\cdot \al^3\be^l \,+\,\\
	 \,+\, \sum_{k,l=1}^\infty \frac18\cdot \al^3 \be^{k+l}  \,+\, \sum_{k=2}^\infty \frac18\cdot \al^3
\be^{k+2^{k-1}-1}.
\end{multline*}
Noting that  $\sum_{k,l=1}^\infty \be^{k+l} = \sum_k \be^k\sum_l\be^l = (\frac{\be}{\al})^2$, after a short calculation  we obtain
$$
	\frac{1}{8}(2+5\al+ \al^3 + 2\be\al^2 + \be + \be^2) + 
        \frac18\al^2\be + \frac18 \al\be^2 +
	\frac18 \al^3\sum_{k=1}^\infty \be^{k+2^{k}},
$$
which is equal to the right-hand side.

Transcendence of  $\sum_{k=1}^\infty (\frac{p-1}{p})^{k+2^{k-1}}$ follows from \cite[Theorem 1]{Tanaka:Transcendence_of_the_values_of_certain_series_with_Hadamard's_gaps}.  Although similar series have
been studied already by Mahler \cite{Mahler:Arithmetische_Eigenschaften_der_Losungen_einer_Klasse_von_Funktionalgleichungen}, the article  \cite{Tanaka:Transcendence_of_the_values_of_certain_series_with_Hadamard's_gaps} seems to be the first
work which implies the transcendence of $\sum_{k=1}^\infty (\frac{p-1}{p})^{k+2^{k-1}}$.
\end{proof}

%~ Now let $p=2$, i.e. $A\rtimes \Ga = \ZZ_2 \wr \ZZ \times (\ZZ_2^3\rtimes \aut(\ZZ_2^3))$,  and $\kk$ be a field of characteristic $q\ge 3$. Let $r$ be the multiplicative order of $2$ mod $q$. Let $L\subset \{2,3,\ldots \}$ be the set of minimal representatives mod $q$ of the powers $2^i$, $i\ge 1$ and for $x\in L$ let $r(x)$ be the smallest such that $2^{r(x)} =x \mod q$.
%~ \luke w introdukcji powiedziec tylko, ze sa wymierne, zbiegaja (ale nie monotnicznie, jesli to prawda), i dac odnosnik do formuly)\lukeend
%~ \begin{cory} 
%~ We have 
%~ $$
%~ \dim_{\kk[A\rtimes \Ga]} \ker \rho(T) = \frac{47}{64} + \frac{1}{128}\scdot \frac{1}{2^r-1} + \frac{1}{64}\scdot \frac{2^q}{2^q-1} \scdot \sum_{x\in L} \frac{1}{2^{x+r(x)-1}}.
%~ %\frac{1}{64}(45+ \frac{1}{2^r -1} + 1 + 2+ 2\sum_{x\in L}\frac{1}{2^{x+r(x)}}\scdot \frac{2^r}{2^r-1}\scdot \frac{2^q}{2^q-1}),
%~ $$
%~ which is a rational number.
%~ \end{cory}
%~ 
%~ \begin{proof}
%~ Rationality of the given number is obvious, since $L$ is finite. 	We analyse the contributions in Theorem \ref{thm:compu-tational-tool} from the graphs of different types. We write $x=y\,\,(q)$ for equalities $\mod q$. 
%~ 
%~ Note that $\mu(\UU) = \frac{45}{64}$. Since $\dim\ker \rho(T_\UU) =1$, this is also the contribution in Theorem \ref{thm:compu-tational-tool}.
%~ 
%~ For the family $\GG$, we compute
%~ \begin{align*}
    %~ \sum_{k\ge 1} \frac{\mu(\supp (\GG(k)))}{|\GG(k)|} \scdot \dim\ker \rho(T_{\GG(k)}) = \sum_{k>1, \,\,2^{k-1}=1(q)}  \frac{1}{64}\scdot\frac{1}{2^k} = 
    %~ \frac{1}{64}\sum_{n=1}^\infty \frac{1}{2^{rn+1}} = \\
    %~ = \frac{1}{128}(\frac{1}{1-2^r} -1) = \frac{1}{128}\scdot \frac{1}{2^r-1}.
%~ \end{align*}
%~ 
%~ For the family $\HH$,
%~ \begin{align*}
    %~ \sum_{l\ge 1} \frac{\mu(\supp (\HH(l)))}{|\HH(l)|} \scdot \dim\ker \rho(T_{\HH(k)}) = \sum_{l\ge 1} \frac{1}{64} \scdot \frac{1}{2^l} = \frac{1}{64}.
%~ \end{align*}
%~ 
%~ Finaly for $\JJ$ we have
%~ \begin{align*}
    %~ &\sum_{k,l\ge 1} \frac{\mu(\supp (\JJ(k,l)))}{|\JJ(k,l)|} \scdot \dim\ker \rho(T_{\JJ(k,l)}) = \frac{1}{64}\sum_{k,l\ge 1} \frac{1}{2^{k+l}}  \dim\ker \rho(T_{\JJ(k,l)})\\
    %~ &\quad = \frac{1}{64}\sum_{k,l\ge 1}   \frac{1}{2^{k+l}} + \frac{1}{64} \sum\limits_{\mathclap{\substack{k,l\ge 1,\\l=2^{k-1}-1\,(q)}}} \frac{1}{2^{l+k}} \,=\, 
    %~ \frac{1}{64} +\frac{1}{64} \sum_{x\in L} \sum_{\substack{n\ge 0\\ m\ge 1}} \frac{1}{2^{(x+qn-1)+ (r(x)\scdot m+1)}} \\
    %~ &\quad =\frac{1}{64} + \frac{1}{64}\sum_{x\in L} \frac{1}{2^x} \scdot \frac{2^q}{2^q-1} \scdot \frac{1}{2^{r(x)}-1} = \frac{1}{64} + \frac{1}{64}\scdot \frac{2^q}{2^q-1} \scdot \sum_{x\in L} \frac{1}{2^{x+r(x)-1}}.
%~ \end{align*}
%~ \end{proof}




